Bug Characteristics in Quantum Software Ecosystem

With the advance in quantum computing in recent years, quantum software becomes vital for exploring the full potential of quantum computing systems. Quantum programming is different from classical programming, for example, the state of a quantum program is probabilistic in nature, and a quantum computer is error-prone due to the instability of quantum mechanisms. Therefore, the characteristics of bugs in quantum software projects may be very different from that of classical software projects. This work aims to understand the characteristics of bugs in quantum software projects, in order to provide insights to help devise effective testing and debugging mechanisms. To achieve this goal, we conduct an empirical study on the bug reports of 125 quantum software projects. We observe that quantum software projects are more buggy than classical software projects and that quantum project bugs are more costly to fix than classical project bugs. We also identify the types of the bugs and the quantum programming components where they occurred. Our study shows that the bugs are spread across different components, but quantum-specific bugs particularly appear in the compiler, gate operation, and state preparation components. The three most occurring types of bugs are Program anomaly bugs, Configuration bugs, and Data type and structure bugs. Our study highlights some particularly challenging areas in quantum software development, such as the lack of scientific quantum computation libraries that implement comprehensive mathematical functions for quantum computing. Quantum developers also seek specialized data manipulation libraries for quantum software engineering like Numpy for quantum computing. Our findings also provide insights for future work to advance the quantum program development, testing, and debugging of quantum software, such as providing tooling support for debugging low-level circuits.

==> Sections/Discussion.tex <==
\section{Discussion} \label{sec:discussion}
%\heng{not sure why performance regression. the performance bug type is related to this instead?}
We have seen in the analysis that most of the bugs in the quantum software ecosystem are program anomalies, configuration bugs, and data type and structure. These bugs can have a serious impact causing the program to crash and leading to poor software quality. Mainly, we observe that quantum programmers have limited or no access to data, matrix, and array manipulation. It is often difficult to implement quantum algorithms, linear algebra routines, error mitigation models, and unitary transformation with the available library working with arrays such as \texttt{Numpy}. This finding suggests that developing \texttt{\textbf{array manipulation tools}} and  dedicated to quantum programming along with a collection of \texttt{\textbf{mathematical algorithms for quantum  and convenience functions}} can prove to be useful to solve a large number of program anomalies and data type and structure bugs.

While exploring the program anomaly bugs, program structural logic bugs happened due to the wrong logical organization of the quantum circuit, state preparation, gate operation, measurement, and state probability expectation computation. These bugs can be avoided by some \texttt{\textbf{automated quantum components and parameter recommendation}} tools. Developing such tools is challenging and opens the door for further research. An approach can be to mine a large-scale code source and extract the common code pattern from experts in order to recommend examples from the most frequent code patterns.

As quantum programs are difficult to debug and quantum components are strongly coupled, \textbf{\texttt{circuit visualization and analysis}} approaches are needed to explore if the circuit has the correct logic structure or if it is the right fit for the problem to solve. This suggestion can resolve the visualization bugs and reduce the program anomaly bugs.

==> lstlisting/compilerDatatype.tex <==
\begin{figure}[!ht]
\captionsetup{type=lstlisting}
\begin{sublstlisting}{\linewidth}

\begin{lstlisting}[language=Python]
backend = StatevectorSimulator()
q = QuantumRegister(1)
qc = QuantumCircuit(q)
# Calling the compile wih the sgd gate causes the code to crash (bug trigger)
qc.sdg(q)
qobj = compile(qc, backend, basis_gates=['u1', 'u2', 'u3'])
\end{lstlisting}
\caption{Trigger of the bug "qiskit compiler (issue Id 2068)"}
\end{sublstlisting}

\begin{sublstlisting}{\linewidth}

\begin{lstlisting}[language=Python, ]
DAGCircuitError: 'not a QuantumRegister instance.
\end{lstlisting}
\caption{Error message}
\end{sublstlisting}

\begin{sublstlisting}{\linewidth}

 \begin{lstlisting}[language=Python]
#Repository:Qiskit/qiskit-terra
#Fix file:  qiskit/extensions/standard/s.py
#Class: SdgGate, method:_define, line:61
rule = [
-            (U1Gate(-pi/2), q[0], [])
+            (U1Gate(-pi/2), [q[0]], [])
        ]
\end{lstlisting}
\caption{Bug fix}
\end{sublstlisting}
\caption{The execution of the code snippet (shown in (a)) triggers an error message (shown in (b)) because the sbg gate definition causes the compiler to crash. The bug fix was passing a list of qubits to the gate definition rule instead of one qubit (as shown in (c)).}
\label{lst:cp_da}
\end{figure}

==> lstlisting/compilerProgramAnomaly.tex <==
\begin{figure}[!ht]
\captionsetup{type=lstlisting}
\begin{sublstlisting}{\linewidth}
\begin{lstlisting}[language=Python]
qc = QuantumCircuit(1, 1)
qc.x(0)
qc.x(0)
# reset function is ignored when the qubit is in the groud state (Triiger the bug)
qc.reset(0)
\end{lstlisting}
\caption{Trigger of the bug "qiskit-terra (issue id 5736 and 5127)"}
\end{sublstlisting}

\begin{sublstlisting}{\linewidth}
\begin{lstlisting}[language=Python]
# cannot compose this gate and raise an error.
if obj.definition is None:
    raise QiskitError('Cannot apply Instruction: {}'.format(obj.name))
if not isinstance(obj.definition, QuantumCircuit):
    raise QiskitError('Instruction "{}" '
QiskitError: 'Cannot apply Instruction: reset'
\end{lstlisting}
\caption{Error message}
\end{sublstlisting}

\begin{sublstlisting}{\linewidth}
 \begin{lstlisting}[language=Python]
#Repository: Qiskit/qiskit-terra
#Fix file: qiskit/dagcircuit/dagcircuit.py
#Class: DAGCircuit, method:_collect_1q_runs, line:1444
-len(s[0].cargs) == 0 and \
+not s[0].cargs and \
not s[0].op.is_parameterized() and \
-isinstance(node.op, Gate):
+isinstance(s[0].op, Gate):
\end{lstlisting}
\caption{Bug fix}
\end{sublstlisting}
\caption{The execution of the code snippet (shown in (a)) triggers the error message (shown in (b)) because when a qubit is already in the ground state the reset function (line 5 in code snippet (a)) is being ignored. The fix was controlling the instance of the gate and properties (as shown in (c))}
\label{lst:cp_pm}
\vspace{-5mm}
\end{figure}

==> lstlisting/gateDataType.tex <==
\begin{figure}[!ht]
\captionsetup{type=lstlisting}

\begin{sublstlisting}{\linewidth}
\begin{lstlisting}[language=Python]
def circuit1(theta, matrix):
    qml.RX(theta, wires=0)
    # Unitary transformation triggers the bug when storing the current values of the quantum function parameters
    qml.QubitUnitary(matrix, wires=1)
    return qml.expval(qml.PauliZ(0)), qml.expval(qml.PauliZ(1))
\end{lstlisting}
\caption{Trigger of the bug "PennyLaneAI (Id 541)"}
\end{sublstlisting}

\begin{sublstlisting}{\linewidth}
\begin{lstlisting}[language=Python]
TypeError: RX: Real scalar parameter expected, got <class 'numpy.complex128'>
\end{lstlisting}
\caption{Error message}
\end{sublstlisting}

\begin{sublstlisting}{\linewidth}
 \begin{lstlisting}[language=Python]
#Repository: PennyLaneAI/pennylane 
#Fix in file: pennylane/qnodes/base.py,
#class:BaseQNode, method:_set_variables(), line: 329
-    Variable.positional_arg_values = np.array(list(_flatten(args)))
+    Variable.positional_arg_values = list(_flatten(args))
\end{lstlisting}
\caption{Bug fix}
\end{sublstlisting}
\vspace{-3mm}
\caption{The execution of the code snippet (shown in (a)) triggers the error message (shown in (b)) because when storing the current values of the circuit with complex arrays, due to NumPy casting rules, a single complex value will cause the entire array to become complex-valued even if the values were originally reals. The bug fix was using a list instead of NumPy array (as shown in (c))}
\label{lst:cp_ga}
\vspace{-5mm}
\end{figure}

==> lstlisting/gateProgramAnomaly.tex <==
\begin{figure}[!ht]
\captionsetup{type=lstlisting}
\begin{sublstlisting}{\linewidth}
\begin{lstlisting}[language=Python]
qc = qk.QuantumCircuit(2)
qc.cx(0, 1)
qc.u1(1e-17, 0)
qc.cx(0, 1)
# Optimize chains of single-qubit gates does not optimize single qubit rotation epsilon (bug triggered in this line)
Optimize1qGatesDecomposition(basis=['u1', 'u2', 'u3'])(qc)
\end{lstlisting}
\caption{Trigger of the bug "qiskit (Id 6473)"}
\end{sublstlisting}

\begin{sublstlisting}{\linewidth}
\begin{lstlisting}[language=Python]
# Repository: Qiskit/qiskit-terra
# Fix in file:qiskit/transpiler/passes/optimization/optimize_1q_decomposition.py
# Class:Optimize1qGatesDecomposition, Method : run(), Line:83
-if np.array_equal(run[0].op.to_matrix(), np.eye(2)):
+if np.allclose(run[0].op.to_matrix(), np.eye(2), 1e-15, 0):
    dag.remove_op_node(run[0])
\end{lstlisting}
\caption{Bug fix}
\end{sublstlisting}
\caption{The execution of the code snippet (as shown in (a)) triggers a wrong gate decomposition operation because it does not optimize single-qubit rotation. The bug was fixed by changing the comparison operator from np.equal to np.allclose (as shown in (b)). "qiskit (Id 6473)"}
\label{lst:go_pa}
\end{figure}

==> lstlisting/measurmentProgramAnomaly.tex <==
\begin{figure}[!ht]
\vspace{-2mm}
\captionsetup{type=lstlisting}
\begin{lstlisting}[language=Python]
#Repository: qiskit/qiskit-aer
N = 12
#Initialize the circuit 
qc = QuantumCircuit(N)
qc.x(range(0, N))
qc.h(range(0, N))
for kk in range(N//2,0,-1):
    qc.ch(kk, kk-1)
for kk in range(N//2, N-1):
    qc.ch(kk, kk+1)
# Measaure the qubit state before compute the expectation value triger the bug
qc.measure_all()
qc.save_expectation_value(Pauli('Z'*12), range(12), label='after_meas_expval')
\end{lstlisting}
\vspace{-2mm}
\caption{The execution of the code snippet returns a different probability expectation state from the awaited result. The bug is triggered because we measure the state before computing the expectation value. The bug fix was to reverse the measure (line 12) and computing the expectation value (line 13) "qiskit-aer (issue id 1334)"\footnote{\url{https://github.com/Qiskit/qiskit-aer/issues/1334}}
}
\label{lst:ms_pa}
\vspace{-3mm}
\end{figure}

==> lstlisting/postProcessingProgramAnomaly.tex <==
\begin{figure}[!ht]
\vspace{-3mm}
\captionsetup{type=lstlisting}
\begin{sublstlisting}{\linewidth}
\begin{lstlisting}[language=Python]
q, c = QuantumRegister(2), ClassicalRegister(2)
circuit = QuantumCircuit(q, c)
circuit.x(q[0])
circuit.measure(q, c)
# to_qiskit : shuffle the order of qubit and causes the bug
converted = to_qiskit(from_qiskit(circuit))

\end{lstlisting}
\caption{Trigger of the bug "mitiq (issue Id 551)"}
\end{sublstlisting}

\begin{sublstlisting}{\linewidth}
\begin{lstlisting}[language=Python]
#Repository: unitaryfund/mitiq
#Fix file:  mitiq/conversions.py, method: _measurement_order, line: 131
def _measurement_order(circuit: qiskit.QuantumCircuit):
    """
    Returns measurements ordered as they appear going left-to-right through the circuit
    """
    order = []
    for (gate, qubits, cbits) in circuit.data:
        if isinstance(gate, qiskit.circuit.Measure):
            order.append((*qubits, *cbits))
    return order
\end{lstlisting}
\caption{Proposed bug fix}
\end{sublstlisting}

\vspace{-3mm}
\caption{The execution of the code snippet (shown in (a)) triggers a bug because he shuffles the order of the qubits when converting from Qiskit to the Cirq circuit. This leads to mixing which ClassicalRegisters correspond to which QuantumRegisters. The bug fix was to add a function to keep the same qubit order during the conversion (shown in (b))}
\label{lst:pst_p_pa}
\vspace{-3mm}
\end{figure}

==> lstlisting/preProcessingDataType.tex <==
\begin{figure}[!ht]
\captionsetup{type=lstlisting}

\begin{sublstlisting}{\linewidth}
\begin{lstlisting}[language=Python]
import numpy as np
import qutip as qt
dat = np.arange(2 * 3 * 3 * 4).reshape((2 * 3, 3 * 4))
qobj = qt.Qobj(dat, dims=[[2, 3], [3, 4]])
# Due to numpy fancy indexing tensors fail to adjust dimensions (Bug trigger)
qt.tensor_contract(qobj, (1, 2)
\end{lstlisting}
\caption{Trigger of the bug qutip (issue id 386)}
\end{sublstlisting}
\vspace{-1mm}

\begin{sublstlisting}{\linewidth}

\begin{lstlisting}[language=Python]
ValueError: total size of the new array must be unchanged
\end{lstlisting}
\caption{Error message}
\end{sublstlisting}
\vspace{-1mm}

\begin{sublstlisting}{\linewidth}

\begin{lstlisting}[language=Python]
#Repository: qutip/qutip
#Fix file: qutip/tensor.py, method: _tensor_contract_single, Line: 362
-return np.sum(arr[sl], axis=0)
+contract_at = i if j == i + 1 else 0
+return np.sum(arr[sl], axis=contract_at)
\end{lstlisting}
\caption{Bug fix}
\end{sublstlisting}
\vspace{-3mm}

\caption{The execution of the code snippet (shown in (a)) triggers a message error(shown in (b)) because the tensor fails to contract out a pair (i,j) when j==i+1 due to NumPy fancy indexing. The bug fix was to define a function to contract a dense tensor along with a single index pair (shown in (c))}
\label{lst:pre_da}
\end{figure}



==> lstlisting/statePreparationDataTyep.tex <==
\begin{figure}[!ht]
\captionsetup{type=lstlisting}
\begin{sublstlisting}{\linewidth}
\begin{lstlisting}[language=Python]
x = enr_destroy([3,3],2)
z = x[0].eigenstates()[1][0]
#  The fock state representation return object with a list of the quantum states with wrong shape which triggers the bug (Z and y are incompatible)
y = enr_fock([3,3],2,[1,1])
\end{lstlisting}
\caption{Trigger of the bug "qutip (issue Id 820)"}
\end{sublstlisting}

\begin{sublstlisting}{\linewidth}

\begin{lstlisting}[language=Python]
#Repository : qutip/qutip
# Fix file: qutip/states.py, Method: enr_fock(), line: 930 
-    return Qobj(data, dims=[dims, 1])
+    return Qobj(data, dims=[dims, [1]*len(dims)])
\end{lstlisting}
\caption{Bug fix}
\end{sublstlisting}
\caption{The execution of the code sipped (shown in (a)) causes a bug because the dimension property (shape) of the fock state representation (line 4 in code snipped (a)) is not compatible with the dimension of z (line 2 in code snipped (a)) and the multiplication of z and y does not work. The bug fix was to adjust the dimension of the fock state representation return object (as shown in (b)) }
\label{lst:sp_da}
\end{figure}

==> lstlisting/statePreparationError.tex <==
\begin{figure}[!ht]
\captionsetup{type=lstlisting}
\begin{sublstlisting}{\linewidth}
\begin{lstlisting}[language=Python]
from qutip import *
D = 13
psi0 = tensor(coherent(D, 100e-9), qeye(D))
# mesolve return wrong error message when passing incompatible dimensions (Bug trigger)
result = mesolve(qeye(D**2), psi0,[0, 100e-9], [destroy(D**2)])
\end{lstlisting}
\caption{Trigger of the bug "qiskit (Id 1456)"}
\end{sublstlisting}

\begin{sublstlisting}{\linewidth}

\begin{lstlisting}[language=Python]
ValueError: operands could not be broadcast together with shapes (28561,) (2197,) 
\end{lstlisting}
\caption{Error message}
\end{sublstlisting}

\begin{sublstlisting}{\linewidth}

\begin{lstlisting}[language=Python]
# Repository: qutip/qutip
# Fix file: qutip/qutip/mesolve.py, method: _test_liouvillian_dimensions, line:320
-if isket(rho0):
-    rho0 = ket2dm(rho0)
+if L_dims[0] != L_dims[1]:
+    raise ValueError("Liouvillian had nonsquare dims: " + str(L_dims))
\end{lstlisting}
\caption{Bug fix}
\end{sublstlisting}
\vspace{-3mm}
\caption{The execution of the code snipped (shown in (a)) correctly raises a message error (shown in b), but the message error content does not reflect the problem. The bug fix was overwriting the error message (as shown in (c))}
\label{lst:sp_er}
\vspace{-5mm}
\end{figure}

==> tables/Git_difficulty.tex <==
\begin{table}[!t]
\centering
%\caption{QSE Topics difficulty}
\vspace{-5pt}
\caption{The difficulty aspect of QSE-related topics on GitHub issues}
\vspace{-4pt}
\begin{tabular}{llrr}
\rowcolor[HTML]{EFEFEF} 
\toprule
                   Topic name &     $\tilde{Hr\,\, to\,\, close}$ &  $\tilde{\#\, comments}$ \\
\midrule
   Data structures and operations &  151.40 &         1 \\
                 Quantum circuits &  114.98 &         1 \\
               Quantum execution results &   98.02 &         1 \\
                 Machine learning &   94.68 &         2 \\
                        API usage &   80.70 &         1 \\
                        Quantum chemistry &   62.89 &         2 \\
    Quantum execution errors &   59.44 &         2 \\
                       API change &   47.34 &         1 \\
                     Algorithm optimization &   39.83 &         1 \\
            Dependency management &   32.40 &         2 \\
                     Unit testing &   28.26 &         1 \\
               Learning resources &   27.02 &         1 \\
          Environment management &   21.57 &         1 \\
\bottomrule
\multicolumn{3}{l}{All the issues are closed at the time we analyzed their status.}
\end{tabular}
\label{table:gitDiff}
\vspace{-7.5mm}
\end{table}

==> tables/QA_taxonomy.tex <==
\begin{table*}[tbp]
\vspace{-2mm}
\caption{A taxonomy of Question Categories which bases on and extends ~\cite{beyer2020kind}}
%\resizebox{\textwidth}{!}{%
\begin{tabular}{llc}
\hline
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{l}{\textbf{Category}} &
  \textbf{Description} &
  \textbf{Freq} \\ \hline
API usage &
  \begin{tabular}[c]{@{}l@{}}Questions of this category are usually identified by ``how to'', i.e., how to use an API or how to implement a functionality.\end{tabular} &
  85 \\ \hline
Theoretical$^{\mathrm{*}}$ &
  \begin{tabular}[c]{@{}l@{}}This category of questioners ask about theoretical explanations of quantum programs, algorithms, and concepts.\end{tabular} &
  54 \\ \hline
Errors &
  \begin{tabular}[c]{@{}l@{}}This category of questions search for explanations and solutions of errors and exceptions when developing\\or executing quantum programs.\end{tabular} &
  49 \\ \hline
Conceptual &
  \begin{tabular}[c]{@{}l@{}}Questions in this category are related to the limitation, background and the underlying concept of an API. \end{tabular} &
  45 \\ \hline
Discrepancy &
  \begin{tabular}[c]{@{}l@{}}Question of this category usually ask for explanations or solutions for unexpected results \\(e.g., ``what is the problem'', ``why not work''.\end{tabular} &
  31 \\ \hline
Learning &
  \begin{tabular}[c]{@{}l@{}}Questions in this category are searching for learning resources such as documentation, research papers, tutorials, or websites.\end{tabular} &
  22 \\ \hline
Review &
  \begin{tabular}[c]{@{}l@{}}This category describes questions like: ``How/Why this is working?'' or ``Is there a better solution?''.\\ Generally, the questions in this category look for a better solution to a problem or for help reviewing the current solution. \end{tabular} &
  17 \\ \hline
Tooling$^{\mathrm{*}}$ &
  \begin{tabular}[c]{@{}l@{}}This category describes questions like ``I am looking for ...'', ``Is there a tool for ...''.\\ These questions search for tools to solve a specific problem or check the features of a tool. \end{tabular} &
  16 \\ \hline
API change &
  \begin{tabular}[c]{@{}l@{}}This category of questions concern about changes of an API and the associated compatibility issues and other implications. \end{tabular} &
  2 \\ \hline
\multicolumn{3}{l}{$^{\mathrm{*}}$Categories newly identified in QSE-related questions.}
\end{tabular}
%}
\label{table:intent}
\vspace{-3mm}
\end{table*}

==> tables/compenent.tex <==
\begin{table*}[]
\caption{Bug distribution across quantum program component}
\vspace{-3mm}
\begin{tabular}{llc}
\hline
\multicolumn{1}{c}{\textbf{Component}} &
  \textbf{Description} &
  \textbf{\begin{tabular}[c]{@{}c@{}}Number of bugs\\ of releases\end{tabular}} \\ \hline
Compiler                     & Translate the quantum program instruction into device level language & 63 \\ \hline
Unitairy transformation &
  A set of operations to alter the state  of the qubit and generate superposition &
  51 \\ \hline
Other                        & Issue related to documentation or we could not label                 & 41 \\ \hline
\begin{tabular}[c]{@{}l@{}}Classical computing and\\ Simulator\end{tabular} &
  Tradition computer component and simulator &
  41 \\ \hline
State preparation            & Is an operation to generate an arbitrary state of a qubit            & 38 \\ \hline
Measurement                   & Measure the final state of a qubit after applying a set of operations & 19 \\ \hline
Post-processing              & Translate the quantum information to classical computer              & 17 \\ \hline
pulse generation and control & Generate and control signal to calibrate qubits                     & 16 \\ \hline
error mitigation             & Final stage of measurement to reduce the state measurement error       & 14 \\ \hline
Quantum cloud access         & Client interface to connect into quantum cloud service provider      & 14 \\ \hline
Visualisation                & Create plot and visualisations                                       & 12 \\ \hline
Pre-processing               & Translate classical data into the quantum program format             & 9  \\ \hline
\end{tabular}
\label{table:compomenet}
\end{table*}

==> tables/difficultyQA.tex <==
\begin{table}[htbp]
\centering
\caption{QSE Topics difficulty}
\begin{tabular}{lrr}
\rowcolor[HTML]{EFEFEF} 
\toprule
                   Topic name &  \% No acc answer &    Hrs to acc answer \\
\midrule
                Quantum similator &              61.19 &  866.10 \\
          Enviremenent management &              58.99 &  120.86 \\
                 Quantum circuits &              58.38 &  128.69 \\
   Data structures and operations &              55.91 &  134.96 \\
                 Quantum execution results &              55.19 &   67.06 \\
               Learning resources &              51.55 &   61.36 \\
 Quantum algorithms understanding &              47.45 &   61.00 \\
            Algorithm compolexity &              46.92 &  345.44 \\
            Dependency management &              37.93 &  107.41 \\
\bottomrule   
\rowcolor[HTML]{EFEFEF} 
\midrule
                       QSE topcis &              52.61 &  210.32 \\
\bottomrule
\end{tabular}
\label{table:QA difficulty}
\end{table}

==> tables/git_topics.tex <==
\begin{table*}[!t]
\vspace{-8mm}
\centering
\caption{QSE-related topics derived from issue reports of quantum computing projects on GitHub} \
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lllll@{}}
\rowcolor[HTML]{EFEFEF} 
\toprule
\multicolumn{1}{c}{\textbf{Manual label}} &
  \multicolumn{1}{c}{\textbf{Keywords}} &
  \multicolumn{1}{c}{\textbf{Description}} &
  \multicolumn{1}{c}{\textbf{\% Freq}} &
  \multicolumn{1}{c}{\textbf{\# Projects}}\\ 
  \midrule
Learning resources &
  \begin{tabular}[c]{@{}l@{}}summary, remove, tutorial, link, documentation\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Search for documentation, tutorials, websites, etc.\end{tabular} &
  14.94  & 109 (90.08\%)\\ \midrule
Environment management &
  \begin{tabular}[c]{@{}l@{}}build, include, library, release, variable\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Development environment and build problems\end{tabular} &
  13.72 & 107 (88.43\%) \\ \midrule
API change &
  \begin{tabular}[c]{@{}l@{}}version, qiskit, code, issue, update\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}API update or deprecation issues\end{tabular} &
  11.65 & 98 (80.99\%) \\ \midrule
Quantum circuits &
  \begin{tabular}[c]{@{}l@{}}gate, circuit, qubit, operation, control\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Elements of quantum circuits (e.g., Qubits, gates) 
  \\and their operations\end{tabular} &
  8.30 & 70 (57.85\%) \\ \midrule
Quantum chemistry &
  \begin{tabular}[c]{@{}l@{}}input, calculation, basis, energy, pyscf\end{tabular} &
   \begin{tabular}[c]{@{}l@{}}Issues with quantum chemistry libraries (e.g., PySCF)\end{tabular} &
  6.72 & 76 (62.80\%)\\ \midrule
Quantum execution errors &
  \begin{tabular}[c]{@{}l@{}}error, artiq, follow, experiment, device\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Errors in the execution of quantum programs\end{tabular} &
  6.38 & 80 (66.12\%)\\ \midrule
Unit testing &
  \begin{tabular}[c]{@{}l@{}}test, check,   fail, unit, script\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Unit  testing failures\end{tabular} &
  6.32 & 87 (71.90\%)\\ \midrule
API usage &
  \begin{tabular}[c]{@{}l@{}}function, method, class, parameter, call\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}How to use an API \end{tabular} &
  5.81 & 80 (66.11\%)\\ \midrule
Quantum execution results &
  \begin{tabular}[c]{@{}l@{}}state, number, result, time, measurement\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Quantum program execution results (i.e., measured state)\end{tabular} &
  5.76 & 89 (73.55\%) \\ \midrule
Data structures and operations &
  \begin{tabular}[c]{@{}l@{}}implement, operator, matrix, problem, array\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Data structures (e.g., matrix, arrays and list) \\and their operations \end{tabular} &
  5.73 & 88 (72.73\%)\\ \midrule
Machine learning &
  \begin{tabular}[c]{@{}l@{}}model, datum, dataset, layer, benchmark\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Quantum computing application in machine learning\end{tabular} &
  5.26 & 75 (61.9\%) \\ \midrule
Dependency management &
  \begin{tabular}[c]{@{}l@{}}file, python, import, package, install \end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Library installation, use and versioning issues \end{tabular} &
  5.23 & 93 (76.86\%) \\ \midrule
Algorithm optimization &
  \begin{tabular}[c]{@{}l@{}}case, time, optimization, long, performance\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}Program performance and algorithm optimization \end{tabular} &
  4.19 & 83 (68.6\%) \\ \bottomrule
\end{tabular}
}
\label{table:git}
\vspace{-5mm}
\end{table*}



==> tables/popularityQA.tex <==
\begin{table}[!t]
\centering
%\caption{Quantum software engineering topics popularity}
\caption{Popularity of QSE-related topics on Stack Exchange forums}
\vspace{-5pt}
\setlength{\tabcolsep}{4.5pt}
\begin{tabular}{lrrr}
\rowcolor[HTML]{EFEFEF} 
\toprule
                   Topic name &   $\tilde{View}$ &   $\tilde{Score}$ & $\tilde{Favorite}$ \\
\midrule
  Quantum vs. classical computing &      147.5 &      3 &            1.5 \\
                 Quantum circuits &      107.0 &      2 &            1.0 \\
           Environment management &      106.0 &      1 &            1.0 \\
               Learning resources &      102.0 &      2 &            1.0 \\
                 Quantum execution results &       98.0 &      1 &            1.0 \\
 Quantum algorithms understanding &       97.5 &      2 &            1.0 \\
            Dependency management &       93.0 &      2 &            1.0 \\
            Algorithm compolexity &       87.5 &      1 &            1.0 \\
   Data structures and operations &       82.0 &      1 &            1.0 \\
\bottomrule
\end{tabular}
\label{table:QA popularity}
\vspace{-5mm}
\end{table}

==> tables/posts.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table*}[htbp]
\vspace{-2mm}
\centering
\begin{tabular}{@{}lccccc@{}}
\cmidrule(l){2-6}
       & \multicolumn{1}{l}{StackOverflow} & \multicolumn{1}{l}{QuantumComputing.stackExchange} & \multicolumn{1}{l}{ai.stackexchange} & \multicolumn{1}{l}{cs.stackexchange} & \multicolumn{1}{l}{Total} \\ \midrule
Post   & 250                               & 1534                                               & 13                                   & 238                                  & 2035                      \\ \midrule
Answer & 183                               & 778                                                & 4                                    & 117                                  & 1082                      \\ \bottomrule
\end{tabular}
\label{table:posts}
\end{table*}

==> tables/statistic_sammary.tex <==
\begin{table*}[]
\tiny
\vspace{-2mm}
\caption{Distribution of the median number of hours, code lines change and files change to fix a bug in a project.}
\begin{tabular}{l|lll|lll|lll|}
\cline{2-10}
 &
  \multicolumn{3}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}median number of hours \\ to fix a bug\end{tabular}}} &
  \multicolumn{3}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Median number of \\ files changed in a commit\end{tabular}}} &
  \multicolumn{3}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Median number of code \\ lines changed in a commit\end{tabular}}} \\ \cline{2-10} 
 &
  \multicolumn{1}{c|}{\textbf{median}} &
  \multicolumn{1}{c|}{\textbf{mean}} &
  \multicolumn{1}{c|}{\textbf{var}} &
  \multicolumn{1}{c|}{\textbf{median}} &
  \multicolumn{1}{c|}{\textbf{mean}} &
  \multicolumn{1}{c|}{\textbf{var}} &
  \multicolumn{1}{c|}{\textbf{median}} &
  \multicolumn{1}{c|}{\textbf{mean}} &
  \multicolumn{1}{c|}{\textbf{var}} \\ \hline
\multicolumn{1}{|l|}{\textbf{Experimental quantum computing}} &
  \multicolumn{1}{l|}{27.98} &
  \multicolumn{1}{l|}{105.51} &
  15,998.01 &
  \multicolumn{1}{l|}{2.00} &
  \multicolumn{1}{l|}{1.75} &
  0.38 &
  \multicolumn{1}{l|}{12.00} &
  \multicolumn{1}{l|}{15.00} &
  100.30 \\ \hline
\multicolumn{1}{|l|}{\textbf{Quantum Machine learning}} &
  \multicolumn{1}{l|}{66.05} &
  \multicolumn{1}{l|}{65.17} &
  2,579.02 &
  \multicolumn{1}{l|}{2.00} &
  \multicolumn{1}{l|}{2.00} &
  1.14 &
  \multicolumn{1}{l|}{38.00} &
  \multicolumn{1}{l|}{61.00} &
  4,364.36 \\ \hline
\multicolumn{1}{|l|}{\textbf{Quantum algorithms}} &
  \multicolumn{1}{l|}{25.01} &
  \multicolumn{1}{l|}{29.26} &
  771.14 &
  \multicolumn{1}{l|}{1.50} &
  \multicolumn{1}{l|}{2.53} &
  9.29 &
  \multicolumn{1}{l|}{15.00} &
  \multicolumn{1}{l|}{1,121.29} &
  22,908,620.00 \\ \hline
\multicolumn{1}{|l|}{\textbf{Quantum circuit simulators}} &
  \multicolumn{1}{l|}{20.61} &
  \multicolumn{1}{l|}{36.78} &
  2,831.37 &
  \multicolumn{1}{l|}{2.00} &
  \multicolumn{1}{l|}{2.41} &
  4.46 &
  \multicolumn{1}{l|}{20.00} &
  \multicolumn{1}{l|}{49.27} &
  7,744.71 \\ \hline
\multicolumn{1}{|l|}{\textbf{Quantum compilers}} &
  \multicolumn{1}{l|}{20.72} &
  \multicolumn{1}{l|}{40.89} &
  2,333.90 &
  \multicolumn{1}{l|}{2.00} &
  \multicolumn{1}{l|}{2.11} &
  0.86 &
  \multicolumn{1}{l|}{28.00} &
  \multicolumn{1}{l|}{32.22} &
  558.88 \\ \hline
\multicolumn{1}{|l|}{\textbf{Quantum programing framework}} &
  \multicolumn{1}{l|}{34.60} &
  \multicolumn{1}{l|}{35.46} &
  1,075.40 &
  \multicolumn{1}{l|}{2.00} &
  \multicolumn{1}{l|}{2.36} &
  1.77 &
  \multicolumn{1}{l|}{30.00} &
  \multicolumn{1}{l|}{44.20} &
  1,859.09 \\ \hline
\multicolumn{1}{|l|}{\textbf{Quantum utility tools}} &
  \multicolumn{1}{l|}{15.40} &
  \multicolumn{1}{l|}{141.60} &
  155,867.74 &
  \multicolumn{1}{l|}{2.00} &
  \multicolumn{1}{l|}{1.63} &
  0.47 &
  \multicolumn{1}{l|}{11.00} &
  \multicolumn{1}{l|}{17.55} &
  469.72 \\ \hline
\multicolumn{1}{|l|}{\textbf{Quantum-based simulation}} &
  \multicolumn{1}{l|}{33.94} &
  \multicolumn{1}{l|}{33.94} &
  375.84 &
  \multicolumn{1}{l|}{2.00} &
  \multicolumn{1}{l|}{2.00} &
  2.00 &
  \multicolumn{1}{l|}{63.00} &
  \multicolumn{1}{l|}{63.00} &
  5,618.00 \\ \hline
\end{tabular}
\label{table:code_change_summary}
\vspace{-3mm}
\end{table*}


==> tables/summary_changes.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[]
\centering
\vspace{-2pt}
\caption{Distributions of Bugs and fixing bug ration over quantum project types.}
\vspace{-4pt}
\begin{tabular}{@{}lcc@{}}
\toprule
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{c}{\cellcolor[HTML]{EFEFEF}\textbf{Programs nature}} &
  \textbf{\begin{tabular}[c]{@{}c@{}}Median number \\ of bugs\end{tabular}} &
  \textbf{\begin{tabular}[c]{@{}c@{}}Median bug fix \\ ratio\end{tabular}} \\ \midrule
\rowcolor[HTML]{FFFFFF} 
Quantum mechanism simulation      & 296.5 & 0.835 \\
\rowcolor[HTML]{FFFFFF} 
Machine learning                  & 759.0 & 0.763 \\
\rowcolor[HTML]{FFFFFF} 
Quantum optimization              & 132.0 & 0.785 \\
\rowcolor[HTML]{FFFFFF} 
Quantum programing Framwork       & 217.5 & 0.852 \\
\rowcolor[HTML]{FFFFFF} 
Quantum simulator                 & 279.0 & 0.721 \\
\rowcolor[HTML]{FFFFFF} 
Post-quantum cryptography         & 201.0 & 0.683 \\
\rowcolor[HTML]{FFFFFF} 
Quantum algorithms                & 170.0 & 0.810 \\
\rowcolor[HTML]{FFFFFF} 
Quantum program quality assurance & 395.0 & 0.769 \\
\rowcolor[HTML]{FFFFFF} 
Language compiler                 & 126.0 & 0.738 \\
\rowcolor[HTML]{FFFFFF} 
Numerical computation             & 155.0 & 0.802 \\
\rowcolor[HTML]{FFFFFF} 
Quantum chemistry                 & 120.0 & 0.805 \\
\rowcolor[HTML]{FFFFFF} 
Quantum physics experiment tool   & 138.0 & 0.841 \\ \midrule
\rowcolor[HTML]{EFEFEF} 
Quantum program                   & 149.0 & 0.793 \\ \midrule
\rowcolor[HTML]{EFEFEF} 
Non-quantum program               &   8.9    &       \\ \bottomrule
\end{tabular}
\label{table:categories}
\vspace{-5pt}
\end{table}

==> tables/tableQAtopics.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[]
\vspace{-8mm}
\centering
\caption{Bugs topics derived from issue reports of quantum computing projects on GitHub} 
\begin{tabular}{@{}llll@{}}
\toprule
\rowcolor[HTML]{EFEFEF} 
Topic Name &
  Key words &
  Description &
  Bug percentage \\ \midrule
\rowcolor[HTML]{FFFFFF} 
Code refactoring &
  current, code, implement, support, user, &
  Bug related to code refactoring and restructing &
  16.3\% \\ \midrule
\rowcolor[HTML]{FFFFFF} 
Dependency management &
  error, version, code, follow, issue &
  Library usage and versioning issues &
  10.6\% \\ \midrule
\rowcolor[HTML]{FFFFFF} 
Data Structures and Operations &
  function, type, return, valu, objec &
  \begin{tabular}[c]{@{}l@{}}Data structures and their operations in\\  quantum programs bugs\end{tabular} &
  9.7\% \\ \midrule
\rowcolor[HTML]{FFFFFF} 
\begin{tabular}[c]{@{}l@{}}Quantum circuit design and \\ optimization\end{tabular} &
  gate, qubit, circuit, measur, oper &
  Circuit design and optimization bugs &
  7.4\% \\ \midrule
\rowcolor[HTML]{FFFFFF} 
Documentation &
  document, updat, exampl, file, link, &
  Bugs related to documentation &
  7.1\% \\ \midrule
\rowcolor[HTML]{FFFFFF} 
Quantum simulators &
  circuit, qiskit, backend, python, result &
  \begin{tabular}[c]{@{}l@{}}Bug related to quantum simulation on \\ classical computing\end{tabular} &
  6.5\% \\ \midrule
\rowcolor[HTML]{FFFFFF} 
Matrix and array operations &
  oper, matrix, state, function, hamiltonian, &
  \cellcolor[HTML]{FFFFFF}\begin{tabular}[c]{@{}l@{}}Quantum unitary transformation and \\ matrix operation bugs\end{tabular} &
  5.6\% \\ \midrule
\rowcolor[HTML]{FFFFFF} 
Quantum chemistry calculation &
  calcul, pyscf, energi, basi, atom, input &
  \begin{tabular}[c]{@{}l@{}}Quantum chemistry , and molecule simulation on\\  Qubits bugs\end{tabular} &
  5.4\% \\ \midrule
\rowcolor[HTML]{FFFFFF} 
Test failure &
  test, fail, build, pass, check, failur &
  Bugs related to testing quantum programs &
  5.1\% \\ \midrule
\rowcolor[HTML]{FFFFFF} 
Installation issues &
  instal, python, version, packag, build &
  Bug reported during installation &
  4.4\% \\ \midrule
\rowcolor[HTML]{FFFFFF} 
Quantum hardware issues &
  artiq, experi, kernel, output, channel &
  Bug in the quantum hardware set up &
  4.4\% \\ \midrule
\rowcolor[HTML]{FFFFFF} 
Compilation errors &
  build, compil, cmake, includ, librari &
  circuit compilation /classical component compilation bugs &
  3.5\% \\ \midrule
\rowcolor[HTML]{FFFFFF} 
Quantum embedding &
  sampl, optim, paramet, return, valu &
  \begin{tabular}[c]{@{}l@{}}Bugs related while mapping data from classical computer \\ to quantum computer\end{tabular} &
  3.2\% \\ \midrule
\rowcolor[HTML]{FFFFFF} 
Infrastructure problem &
  node, error, time, connect, memori &
  Memory leak problem and excution bugs &
  3.1\% \\ \midrule
\rowcolor[HTML]{FFFFFF} 
Machine learning &
  model, dataset, deepchem, train, featur, &
  Bugs related to quantum machine learning &
  2.5\% \\ \midrule
\rowcolor[HTML]{FFFFFF} 
Envirement setup errors &
  file, import, error, python, init, modul, &
  Envirenment development and build bugs &
  2.4\% \\ \midrule
\rowcolor[HTML]{FFFFFF} 
\begin{tabular}[c]{@{}l@{}}Building and measurment of \\ pulse scheduler\end{tabular} &
  pul, schedul, measur, instruct, sequenc &
  Bugs in quantum pulse regulation and Qubits callibration &
  2.3\% \\ \bottomrule
\end{tabular}
\label{table:Topics}
\end{table*}
